Natural Language Querying System Through Entity Enrichment

This paper focuses on a domain expert querying system over databases. It presents a solution designed for a French enterprise interested in offering a natural language interface for its clients. The approach, based on entity enrichment, aims at translating natural language queries into database queries. In this paper, the database is treated through a logical paradigm, suggesting the adaptability of our approach to different database models. The good precision of our method is shown through some preliminary experiments.

==> NLQ-backG.tex <==

We use a logical paradigm to express RDF databases  and queries.
Thus, we write $C(a)$  (instead of the triple-format  \textsf{(a rdf:type C)}) to express that $a$ is an instance of class $C$  and
$P(a,b)$ to express that $a$ has value $b$ for property $P$
(instead of \textsf{(a P b)}).
For instance, \textsf{Doctor(Bob)}  and \textsf{writtenBy(Urgency Service, Bob)}.

%\textsf{Doctor(Kaplan)} to express that \textsf{Kaplan} is an instance of class \textsf{Doctor} 
%(the corresponding  triple-format  is \textsf{Kaplan rdf:type Doctor})
%and we write
%\textsf{writtenBy(Lost after translation, Kaplan)} to expresses 
%the fact that \textsf{Lost after translation} has \textsf{Kaplan} as value for property \textsf{writtenBy}
%(\ie, \textsf{(Lost after translation, writtenBy, Kaplan)} in the triple-format).

Formally, we consider  disjoint countably infinite sets of constants ({\sc const}) and
variables ({\sc var}) and a finite set of predicates ({\sc pred}).
As we deal with RDF, predicates are of arity one  or two.
A term is a constant or a variable.  
 An  {\em atom} has  one of the forms:
 ($i$) $P(t_1, . . . , t_n)$, where $P$ is an $n$-ary predicate and $ t_1 , . . . , t_n$ are terms;
($ii$) $\top$ (true) or $\bot$ (false);
%($iii$) $(t_1 ~op~  t_2)$, where $t_1$ and $t_2$ are terms and
 % $op$ is  a comparison operator (=, $<$, $>$, $\leq$, $\geq$).
 ($iii$) $(t_1 ~op~  \alpha_2)$, where %$\alpha_1$ and $\alpha_2$
 $t_1$ is a  term,  %($t_1$ and  $t_2$) 
 $\alpha_2$ is a term
 or    a character string,  % ($str_1$ and $str_2$) %(\ie, $\alpha = h(str)$) 
 and $op$ is  a comparison operator such as $=$, $<$, $>$, $\leq$, $\geq$ or an operator for comparing strings namely, \textit{startingWith},
 \textit{endingWith}.
  A \textit{fact}
is  an  atom  $P(u)$ where $ u \in  $({\sc const})$ ^n$.  
A \textit{database schema} is defined by a set of predicates \Sch\ and a \textit{database instance} is a set of facts (denoted by \db) on \Sch.

Let $A_1$ and $A_2$ be a set of atoms. A \textit{homomorphism} from  an atom in $A_1$ to an atom in $A_2$ both on the same  predicate $P$, is a function $h$ from the  terms of $A_1$ to  the  terms of $A_2$ such that:
($i$) if $t\in $ {\sc const}, then $h(t)= t$, and 
($ii$) if $P(t_1,...,t_n) \in A_1$, then $P(h(t_1), . . . , h(t_n)) \in A_2$. 
This notion  extends to conjunctions or  sets of atoms.
A \textit{(conjunctive) query}  $q$  over  a given schema
has the rule-form
$R_0 (u_0) \leftarrow R_1(u_1) \dots  R_n(u_n), comp_1, \dots, comp_m$
where $n \geq 0$, $R_i$ ($0 \leq i \leq n$) are predicate names,  $u_i$ are  free tuples (\ie, a tuple of terms) of 
appropriate arity and $comp_j$  ($0 \leq j \leq m$) are comparison formulas involving variables appearing in at least one free tuple from $u_1$ to $u_n$.
We denote $head(q)$ (respect. $body(q)$)  the expression on the left hand-side (respect. right hand-side) of $q$ .
Conjunctive queries are,  as usual, range restricted and satisfiable~\cite{AHV95}.
Denote $ans(q, \db)$ the set of answers (tuples) $t \in \textsc{const}^n$ for which  $\exists h_t$ such that
$\{h_t(R_1(u_1)),  \dots,  h_t(R_n(u_n))\} \subseteq \db$,  the conjunction of all $h_t(comp_j)$ is evaluated to true
(according to the usual semantic of opertors $op$) and $h_t(u_0)= t$.
In this rule-based formalism, the union is expressed by allowing more than one rule with the same head.
For instance, 
$q(X) \leftarrow writtenBy(X, Bob)$ together with
$q(X) \leftarrow editedBy(X, Bob)$
express a query looking for documents written or edited by \textit{Bob}.




==> NLQ-sysOverview.tex <==
\mhf{I am writing some explanations here but I do not know yet how the paper beginning is going to be restructured. Perhaps we do not need a section...  to be seen how to compose with the introduction}

Our querying system is available over an RDF database storing  information about medical documents.
The system  translates a natural language query (NL-query) into a database query (DB-query) offering a user-friendly interface.


Our motivation is to allow a user to perform the so-called \textit{facet search},   narrowing down search results by applying multiple filters.
Accepted queries are those  requiring information on instances of one unique class (denoted here as solar-class).
The image comes from an RDF graph where a node is an instance of a class and edges are associated to the node's properties or relationships with other nodes.
Our queries are built over an RDF  schema which can be draw as a sun: the class (the node) and the properties having the class as domain or range (the edges).
The allowed query is the one that wants to identify nodes respecting some conditions among those that belong to a given class
For instance, supposing our solar-class is \textit{Book} the query requiring book instances edited by doctor Alice is considered.
If the user wants to identify doctors who are writers, then he has, firstly, to change  his solar-class specification.
In other terms, our query are simple queries (translated into conjunctive database queries)  identifying instances of one class (even if it can also renders some properties of these instances). The  NL-query follows the format \textit{Find books which...} (establishing Book as the solar-class), \textit{Find doctors who...}
(Doctors as the solar-class), etc.


The following example introduces our running example. We will use it in the rest of the paper in order to show, step by step, how we transform a NL-query into a DB-query. 


%We decide to use only entity extraction and resolution instead of using a translation model as in \cite{wangCrossdomainNaturalLanguage2019}.
%This decision is justified by the fact that we have a limited vocabulary and knowledge.
%To find facets, you must resolve the entities (\ie map a named entity value to a database ID or a literal.) but also typed it correctly to retrieve the facet name.

\begin{example}
\label{ex:introRunEx}
Let \db\ be an RDF database instance over a given schema \Sch. In the rest of this paper we will denote the query of our running example
as $Q_{run}$. It come in two flavours. The  NL-query, denoted by $NLQ_{run}$ is:
\vspace{-0.1cm}
\small
\begin{quote}
\textit{Find books with title "Principle of Medicine" co-authored by Bob and Alice and whose price is less tan 30 dollars.}
\end{quote}
\normalsize
\vspace{-0.1cm}
\textit{Book} is  our solar-class and  thus the DB-query should return the identifiers of book instances. 
The query should also include all the  conditions imposed on the books being selected.
The following conjunctive DB-query (expressed in a logical formalism) is the $DBQ_{run}$:

\vspace{-1em}
\small
\begin{equation*}
	\begin{split}
		q(x) \leftarrow & Book(x), asTitle(x, "Princ. ~of ~Medecine"), Person(y_1),\\
		& writtenBy(x, y_1), Person(y_2), writtenBy(x, y_2), asPrice(x, y_3),\\
		& (y_1 = \text{:bob}), (y_2 = \text{:alice}), (y_3 < 30)\\
	\end{split}
\end{equation*}
\normalsize

\end{example}
